Network information theory for classical-quantum channels

Network information theory is the study of communication problems involving multiple senders, multiple receivers and intermediate relay stations. The purpose of this thesis is to extend the main ideas of classical network information theory to the study of classical-quantum channels. We prove coding theorems for quantum multiple access channels, quantum interference channels, quantum broadcast channels and quantum relay channels. A quantum model for a communication channel describes more accurately the channel's ability to transmit information. By using physically faithful models for the channel outputs and the detection procedure, we obtain better communication rates than would be possible using a classical strategy. In this thesis, we are interested in the transmission of classical information, so we restrict our attention to the study of classical-quantum channels. These are channels with classical inputs and quantum outputs, and so the coding theorems we present will use classical encoding and quantum decoding. We study the asymptotic regime where many copies of the channel are used in parallel, and the uses are assumed to be independent. In this context, we can exploit information-theoretic techniques to calculate the maximum rates for error-free communication for any channel, given the statistics of the noise on that channel. These theoretical bounds can be used as a benchmark to evaluate the rates achieved by practical communication protocols. Most of the results in this thesis consider classical-quantum channels with finite dimensional output systems, which are analogous to classical discrete memoryless channels. In the last chapter, we will show some applications of our results to a practical optical communication scenario, in which the information is encoded in continuous quantum degrees of freedom, which are analogous to classical channels with Gaussian noise.

==> 08.a.Quantum-optics-intro.tex <==

Bosonic Channels 

The most commonly used quantum communication channel is the
so-called bosonic channel with Gaussian noise and loss [40]. Bosonic channels
are ones that use bosons such as photons or phonons to communicate. Gaussian
noise and loss is the most common type of noise and loss for such channels, it
includes the effect of thermal noise, noise from linear amplification, and
leakage of photons or phonons out of the channel. It has been shown that the
capacity for bosonic channels with loss alone is attained by sending coherent
states down the channel [42]. Coherent states are the sort of states produced
by lasers and are the states that are currently used in most bosonic channels.
It has been conjectured that coherent states also maximize the capacity of
quantum communication channels with Gaussian noise as well as loss [43]. This
conjecture, if true, would establish the quantum-mechanical equivalent of
Shannon’s theorem for the capacity of classical channels with Gaussian noise
and loss. The resolution of this conjecture can be shown to be equivalent to
the following, simpler conjecture: 

Gaussian Minimum Output Entropy Conjecture:

Coherent states minimize the output entropy of bosonic channels with Gaussian
noise and no loss.  The Gaussian minimum output entropy is intuitively
appealing: an equivalent statement is that the vacuum input state minimizes
the output entropy for a channel with Gaussian noise. In other words, to
minimize the output entropy of the channel, send nothing.  Despite its
intuitive appeal, the Gaussian minimum output entropy conjecture has
steadfastly resisted proof for decades. This conjecture is related to the
additivity conjectures above: in particular, if the additivity conjectures
can be shown to be true, then the Gaussian minimum output entropy conjecture
is also true [110]. It is not known whether the converse implication also
holds. Proving the additivity conjectures and the Gaussian minimum output
entropy conjecture is one of the primary goals of quantum information theory.


FROM:
Quantum Information Processing -- introductory article by Seth Lloyd.pdf


==> 10.A.3_Strong_classical_typicality.tex <==


%!TEX root = thesis.tex



\section{Strongly typical sequences}
											\label{apdx:strong-typicality}
							

	Most of the result sin this thesis can use entropy-typical sequences sets
	or letter-typical sequences.
	
	These are CS or PHYSICS view of probabilities...
	
	The results the Marton coding scheme depend on strongly typical sets
%	
%	we review
	
					
	%	Consider the probability distribution $p_{X}(x)$ on the set $\cX$.
	%	Define the probability distribution $p_{X^n}(x^n)$ on $\cX^n$ to be the
	%	$n$-fold product of $p_{X}$. 
	%	The sequence $x^n$ is drawn from $p_{X^n}$ if
	%	and only if each letter $x_i$ is drawn independently from $p_X$.
	For any $\delta >0$,	define the set of $\delta$-typical sequences of length 
	$n$ as $\cT^{n}_{p,\delta}$, as
	\be
		\cT^{n}_{p,\delta} 
		\equiv 
		\left\{ 
			x^n \in \mcal{X}^n \ \big| \ |(t_\alpha)_a -p_X(x_a)| \leq \delta, \ \forall x_a\in\cX 
		\right\}.
	\ee
	%
	Furthermore define the set of \emph{typical types} $\mathbf{\tau}_\delta \subseteq \mathbf{t}$ as
	\be
		\mathbf{\tau}_\delta
		\equiv 
		\left\{
			t_\alpha \in \mathbf{t} \ \big| \ | (t_\alpha)_a-p_X(x_a)|\leq \delta, \ \forall x_a \in \cX
		\right\}.
	\ee
	We can write the set of typical set as union over the sequences in the typical types
	\be	\label{eqn:uni-over-types}
			\cT^{n}_{p,\delta} =\underset{t_\alpha \in \tau_\delta}{\bigcup} {\top_{\!\!\alpha}}.
	\ee
	%
	% not used anywhere....
	%$|\tau_\delta|=a$.

	
	Typical sequences enjoy many useful properties \cite{CK81}.
	Let $H(p)	= - \sum_x p_X(x) \log p_X(x)$ be the Shannon entropy of $p_X$. 
	For any $\epsilon,\delta>0$, and all sufficiently large $n$, we have
	\begin{eqnarray}
		& 
		p_{X^n}\!\!\left(\cT_{p,\delta}^{n} \right)  
		& \geq  1-\epsilon,   \label{cc1}  \\
		%
		2^{-n[ H(p)+\delta ]}  \leq &
		p_{X^n}(x^n) & 
		\leq   2^{-n[H(p)-c\delta]}  \ \ \  \forall x^n \in \cT_{p,\delta}^{n} 
		\label{cc2} \\
		%
		(1 - \epsilon)^{-1}  2^{n[ H(p)-c\delta]} \leq &  
		|\cT_{p,\delta}^{n}| 
		& \leq 2^{n[ H(p)+c\delta]}, \label{cc3} 
	\end{eqnarray}
	for some constant $c$. 
	
	
	For $t_\alpha \in \tau_\delta$ and for
	sufficiently large $n$, the cardinality $d_{\alpha}$ of ${\top_{\!\!\alpha}}$ is
	bounded as
	%$|{\top_{\!\!\alpha}}| = D_t$.
	\be 	\label{cc4} 
		d_\alpha \geq 2^{n [H(p) - c\delta - \eta(\delta)]}, \ \ \ \text{for } t_\alpha \in \tau_\delta,
	\ee 
	where $c$ is a constant and the function $\eta(\delta) \rightarrow 0$ as $\delta \rightarrow 0$.
	%	\comment{it seems to contradict (\ref{eqn:uni-over-types}) -- how can each
	%			type subspace have roughly $2^{nH(p)}$ elements and the total number
	%			of elements typical sequences be $ \leq 2^{n[ H(p)+c\delta]}$ 
	%			as stated in (\ref{cc3}) ? }
	% ANSWER: http://markwilde.com/teaching/notes/ch-13-classical-typicality.pdf page 307
	%Let $\alpha=\sum_{x^n\in\cT^{n}_{p,\delta}}p_{x^n}$.
	%From (\ref{cc1}), we have $\alpha\geq 1-\epsilon$.
	%Define $\pt$ as the normalized probability that type $t$ in the set
	%$\tau_\delta$ occurs:
	%$$
	%\pt=\frac{\sum_{x^n\in{\top_{\!\!\alpha}}}p^n(x^n)}{\sum_{x^n\in\cT^{n}_{p,\delta}}p^n(x^n)}.
	%=\frac{1}{\alpha}\sum_{x^n\in\cT_{t}}p_{x^n}
	%$$
	%Clearly $\sum_{t\in\tau_\delta}\pt=1$.


[FIXME] joint typical implied ... Marton needs what???






==> 11.B.2_Useful_lemmas.tex <==



%!TEX root = thesis.tex


\section{Useful lemmas}





	Finally, we state this useful lemma: 
	% for gentle measurement on ensembles:
		
		%%% MOVED TO HSW THM PROOF SECTION
		\begin{lemma}[Gentle Operator Lemma for Ensembles \cite{itit1999winter,ON07}]
					%\label{lem:gentle-operator}
		Given an ensemble $\left\{  p_{X}\left(  x\right)  ,\rho_{x}\right\}  $ with
		expected density operator $\rho\equiv\sum_{x}p_{X}\left(  x\right)  \rho_{x}$,
		suppose that the operator $\Lambda$ such that $0 \leq \Lambda\leq I$ succeeds
		with high probability on the state $\rho$:%
		\[
		\text{Tr}\left\{  \Lambda\rho\right\}  \geq1-\epsilon.
		\]
		Then the subnormalized state $\sqrt{\Lambda}\rho_{x}\sqrt{\Lambda}$ is close
		in expected trace distance to the original state $\rho_{x}$:%
		\[
		\mathbb{E}_{X}\left\{  \left\Vert \sqrt{\Lambda}\rho_{X}\sqrt{\Lambda}%
		-\rho_{X}\right\Vert _{1}\right\}  \leq2\sqrt{\epsilon}.
		\]

		\end{lemma}
		
		
		
		
		
		%%% MOVED TO BACKGROUND CHAPTER 
		\begin{lemma}
%															\label{lem:trace-inequality}
		Let $\rho$ and $\sigma$ be positive operators and
		$\Lambda$ a positive operator such that $0\leq\Lambda\leq I$. Then the
		following inequality holds%
		\[
		\text{Tr}\left\{  \Lambda\rho\right\}  \leq\text{Tr}\left\{  \Lambda
		\sigma\right\}  +\left\Vert \rho-\sigma\right\Vert _{1}.
		\]
		\end{lemma}




	HAYASHI NAGAOKA
	
%	cite:
%	Masahito Hayashi and Hiroshi Nagaoka. General formulas for capacity of classical-quantum channels. IEEE Transactions on Information Theory, 49(7):1753Ð1768, 2003.
%	= 0206186v4.pdf
	
		%%% MOVED TO HSW THM PROOF SECTION
		\begin{lemma}[Hayashi-Nagaoka \cite{hayashi2003general}] 
															%\label{lem:HN-inequality}
		If $S$ and $T$ are operators such that  
		%	The Hayashi-Nagaoka operator inequality applies to a positive operator 
		%	$T$ and
		%	an operator $S$ where 
		$0\leq T$ and $0\leq S\leq I$, then
		\be
			I-\left(  S+T\right)  ^{-\frac{1}{2}}S\left(  S+T\right)  ^{-\frac{1}{2}}%
			\ \: \leq \ \:
			2\left(  I-S\right) \  + \ 4T.
		\ee
		\end{lemma}%
		

